Raising the Bar in Graph OOD Generalization: Invariant Learning Beyond Explicit Environment Modeling

Out-of-distribution (OOD) generalization has emerged as a critical challenge in graph learning, as real-world graph data often exhibit diverse and shifting environments that traditional models fail to generalize across. A promising solution to address this issue is graph invariant learning (GIL), which aims to learn invariant representations by disentangling label-correlated invariant subgraphs from environment-specific subgraphs. However, existing GIL methods face two major challenges: (1) the difficulty of capturing and modeling diverse environments in graph data, and (2) the semantic cliff, where invariant subgraphs from different classes are difficult to distinguish, leading to poor class separability and increased misclassifications. To tackle these challenges, we propose a novel method termed Multi-Prototype Hyperspherical Invariant Learning (MPHIL), which introduces two key innovations: (1) hyperspherical invariant representation extraction, enabling robust and highly discriminative hyperspherical invariant feature extraction, and (2) multi-prototype hyperspherical classification, which employs class prototypes as intermediate variables to eliminate the need for explicit environment modeling in GIL and mitigate the semantic cliff issue. Derived from the theoretical framework of GIL, we introduce two novel objective functions: the invariant prototype matching loss to ensure samples are matched to the correct class prototypes, and the prototype separation loss to increase the distinction between prototypes of different classes in the hyperspherical space. Extensive experiments on 11 OOD generalization benchmark datasets demonstrate that MPHIL achieves state-of-the-art performance, significantly outperforming existing methods across graph data from various domains and with different distribution shifts.

==> 1_intro/intro_v1.tex <==
% Graph Neural Networks (GNNs) have made significant progress in processing unstructured data such as social networks, material graphs and molecules, showing the state-of-the-art performance, and are widely used in molecular property prediction, drug discovery and other fields. Its core is to encode node features and graph structure information through a message passing mechanism, and then pool the embedding of nodes or edges to generate a global vector of the graph and apply it to downstream tasks. However, the success of GNNs is often based on the assumption that the training and testing sets are independent and identically distributed, which is difficult to hold when deploying models to real-world scenarios. 
% Several studies have shown that GNNs tend to perform poorly on Out-of-distribution (OOD) data, which can significantly compromise their robustness and security. For instance, in molecular property prediction, such as determining toxicity, a well-trained GNNs may perform well on the known training distribution. However, in real-world scenarios, molecules with novel scaffolds or sizes, unseen in the training data, are inevitable. It is crucial that the model maintains its performance when encountering such data to mitigate potential safety risks.

Graph Neural Networks (GNNs) have made remarkable advancements in processing unstructured data, including social networks, material graphs, and molecules. These models have achieved state-of-the-art performance and are widely applied in tasks such as molecular property prediction and drug discovery. At the core of GNNs lies a message-passing mechanism, which encodes both node features and graph structure information. By aggregating node or edge embeddings, GNNs generate a global representation of the entire graph, which is then used for downstream tasks. However, this success is often built on the assumption that training and testing data are independent and identically distributed (IID), an assumption that rarely holds in real-world applications.

In practice, deploying GNNs in real-world scenarios reveals their vulnerability when faced with Out-of-Distribution (OOD) data. Several studies have demonstrated that GNNs often struggle to maintain performance when tested on data that differ significantly from the training set, which raises concerns about the models' robustness and security. For example, in molecular property prediction tasks, models may encounter molecules with novel scaffolds or sizes that were not part of the training distribution. Similarly, in social network analysis, the underlying graph structure could change due to the emergence of new communities or interactions, leading to unexpected behavior. These variations in data distributions, common across domains, highlight the need for models to perform consistently under OOD conditions to mitigate potential risks and ensure reliable outcomes.

Most recent research on graph OOD generalization has focused on invariant learning methods. These approaches aim to capture stable relationships between features and labels that remain consistent across different environments. By leveraging the principle of invariance, these methods enable the model to generalize effectively under distribution shifts. Typically, such methods assume the presence of environment labels during training, which facilitates the learning of these invariant relationships and allows for better OOD generalization performance.  This line of thinking originates from the computer vision (CV) field, where environment labels, such as background or image style, are often available or easily inferred.
In the context of graph data, accurately defining and distinguishing environments presents a fundamental challenge. Unlike images, which allow for clear segmentation based on visual cues, graphs inherently lack explicit structural boundaries, complicating the identification of distinct environments. This complexity poses a critical question: \textbf{Can we truly rely on these predefined environments, or is there a better way to achieve robust OOD generalization in graphs?}

Beyond the challenge of environment definition, another key obstacle is the \textbf{semantic cliff}, which affects the separability of invariant subgraphs. As illustrated in Figure 1, synthetic datasets like house and cycle suggest that identifying the invariant subgraph could allow effective classification. However, in practice, this task becomes difficult unless the dataset's structure is already known, allowing for targeted method design.
For example, in molecular graphs, a functional group often serves as the invariant subgraph. Even slight alterations, such as changing a single atom or bond, can drastically impact a molecule's properties or classification. This variability complicates the identification of invariant subgraphs that consistently map to the same class, particularly when working with unknown or novel datasets.

In this paper, we approach these two challenges from a fundamentally new perspective, one that shifts away from traditional reliance on predefined environments or explicit subgraph extraction. Instead of directly working with the raw graph structures or assuming the availability of environment labels, our method focuses on extracting invariant representations in the GNN-encoded latent space. This allows us to bypass the inefficiencies and limitations associated with environment-based partitioning and manual subgraph identification, offering a more flexible and generalizable solution to the OOD generalization problem in graphs.

Instead of relying on predefined environments or manually extracted subgraphs, our method introduces a novel approach to OOD generalization by focusing on invariant feature extraction in the GNN-encoded latent space. These features are projected into a unit-norm hyperspherical space, where the distances between class prototypes drive classification. To ensure robustness, we introduce two loss functions: the Invariant Feature Loss (IFL), which promotes stability in the learned features across different data distributions, and the Separation Loss (SL), which encourages clear differentiation between classes, even under unseen distribution shifts. These losses are designed to work synergistically, aligning the learned representations with the underlying structure of the graph data while maintaining generalization performance across varying distributions.


The main contributions of this paper are as follows:

\begin{itemize}[leftmargin=*]
    \item \textbf{Novel OOD Generalization Framework for Graphs}: We propose a new approach to graph OOD generalization by focusing on invariant feature extraction in the latent space of GNNs. This method bypasses the reliance on predefined environments or explicit subgraph extraction, offering a more flexible and scalable solution.
    
    \item \textbf{Hyperspherical Representation and Loss Functions}: We introduce a hyperspherical representation space for graph classification, along with two new loss functions—\textit{Invariant Feature Loss (IFL)} and \textit{Separation Loss (SL)}. These losses are specifically designed to ensure robustness against distribution shifts and improve the generalization capability of the model.
    
    \item \textbf{Theoretical Consistency and Empirical Validation}: We provide a detailed theoretical analysis demonstrating that our proposed losses align with the goals of robust OOD generalization. Additionally, our method is validated through extensive experiments on the DrugOOD and GOOD benchmarks, where it consistently outperforms existing methods.
\end{itemize}



% \colorbox{lightgray}{\begin{varwidth}{\linewidth}\textit{
% % Can we truly rely on these predefined environments, or is there a better way to achieve robust OOD generalization in graphs?
% How do we effectively capture stable patterns in graph data, when there are no clear\\ visual  cues or well-defined boundaries to guide the extraction of invariant features?}\end{varwidth}}

% However, unlike Euclidean data, graphs are complex and highly abstract non-Euclidean structures, which present two key challenges for out-of-distribution generalization: 1) \textit{Defining and partitioning environments effectively is difficult}. In computer vision, datasets can be manually divided into multiple subsets based on background or image style, but it is challenging or even infeasible for graphs since we don't have a clear and reasonable defination of the environment of a graph. Consequently, existing graph OOD methods based on invariant learning often fail to match the performance predicted by theoretical analysis, as they lack accurate environment information. 2) \textit{The 'semantic cliff' in graphs results in poor separability of the  invariant subgraph}. Even when invariant subgraph are identified across environments, they tend to be fragile and indivisible. For example, in molecular graphs, the invariant subgraph is typically a functional group conresponding to labels, but a change in just one atom or bond (represented by nodes and edges) can lead to drastic shifts in the molecule's properties or label. As a result, two seemingly similar invariant subgraphs may correspond to entirely different classes or attributes, which defeats the purpose of invariant learning (similar invariant subgraphs should have the same class).


% In this paper, we address these two problems from a new perspective, distinct from existing approaches. Our goal is to design an algorithm that ensures representations from different environments but with the same label exhibit maximal similarity, while representations with different labels, regardless of their environment, maintain maximal separability. In other words, we aim to maximize intra-class invariance and inter-class separability. To achieve this, we first perform invariant feature extraction in the GNN-encoded latent space, avoiding the inefficiency of directly extracting invariant subgraphs from the original graph. We then map the invariant features to a unit norm hyperspherical space for classification by comparing the distances between and the class prototypes. We propose two types of loss functions: $L_{intra-inv}$ which ensures intra-class feature invariance without requiring environmental information, and $L_{inter-sep}$ which maximizes class-based separability of the extracted invariant features. We provide a detailed theoretical analysis to demonstrate the consistency of our loss functions with the proposed objective. In terms of empirical performance, our experimental results on two graph OOD generalization benchmarks, DrugOOD and GOOD, validate the effectiveness of our method. The main contributions of this paper are as follows:

% \begin{itemize}
%     \item We first propose the OOD generalization method for graphs based on hyperspherical representation learning. Invariant feature extraction is conducted in the encoded latent space, and distance-based classification is performed in the unit hyperspherical space. Intra-class invariance and inter-class separability are ensured through the optimization of $L_{intra-inv}$ and $L_{inter-sep}$.
%     \item We provide a detailed theoretical analysis proving the consistency between our proposed loss functions and the objective of achieving OOD generalization.
%     \item Experimental results on the DrugOOD and GOOD benchmarks validate the effectiveness of our approach.
% \end{itemize}
%第一个：推导出这个理论框架，Eq 6
%第二个： 理论基础上，实现方法本身
%第三个： 实验



% To address the challenges of environment capturing and the semantic cliff, we propose a novel framework that combines \textbf{prototype-based invariant learning} with a \textbf{hyperspherical embedding space}. Our approach bypasses the need for explicit environment modeling by introducing prototypes as implicit representations of environment variants. This allows the model to extract robust invariant features across varying environments without relying on environment labels. To further enhance the class separability and ensure the model's robustness, we introduce two key loss functions: \ding{172} \textit{Invariant Prototype Matching Loss ($\mathcal{L}_{IPM}$)}  ensures that samples from the same class are assigned to the same class prototypes, acting as positive samples. In contrast, samples incorrectly assigned to these prototypes—due to environmental influences—are treated as negative samples, driving the model to improve its invariance to environment-induced variations. \ding{173} \textit{Prototype Separation Loss ($\mathcal{L}_{PS}$)}  optimizes the relationship between prototypes, making sure that prototypes belonging to the same class are similar, while those from different classes remain dissimilar. By refining the inter-class boundaries in hyperspherical space, this loss enhances the discriminative power of the model, thereby reducing the impact of the semantic cliff.
 %sx:我认为在latent space 提取不变特征不是很重要的创新，主要的创新还是首次将图不变学习和超球空间结合，利用超球空间中prototype的特性，保证在无环境信息的情况下学习到满足不变性的表征（对应挑战1）并提升可分性（挑战2）

% The main contributions of this paper are as follows:

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Integration of Invariant Learning with Hyperspherical Embedding:} We introduce a novel framework that combines graph invariant learning with hyperspherical embedding, enabling robust invariant representation learning without explicit environment labels.
    
%     \item \textbf{Prototype-Based Implicit Environment Representation: } By leveraging multi-prototypes to represent implicit environment variants, our method addresses the challenge of environment capturing in graph data, eliminating the need for explicit environmental modeling.
    
%     \item \textbf{Novel Loss Functions for Invariance and Separability:}  We propose two key loss functions: the Invariant Prototype Matching Loss to enhance invariance, and the Prototype Separation Loss to improve inter-class separability, effectively addressing the semantic cliff problem and improving OOD generalization.
% \end{itemize}


==> 1_intro/intro_v2.tex <==
Graph Neural Networks (GNNs) have made remarkable advancements in modeling and learning from graph-structured data across various scenarios, including, but not limited to, social networks~\citep{fan2020graph,chang2021sequential}, molecules~\citep{shui2020heterogeneous,liu2024data}, and knowledge graphs~\citep{kg_1,kg_2}. Despite the powerful representational capabilities of GNNs, their success often relies on the assumption that the training and testing data follow the same distribution. Unfortunately, such an assumption rarely holds in most real-world applications, where out-of-distribution (OOD) data from different distributions often occurs~\citep{OODsurvey}. Empirical evidence has shown that GNNs often struggle to maintain performance when tested on OOD data that differ significantly from the training set~\citep{OODbench,li2022ood}. These vulnerabilities underscore the critical need to enhance the OOD generalization capabilities of GNNs, which has become a rapidly growing area of research~\citep{good,drugood}.

Building on the success of invariant learning in addressing OOD generalization challenges in image data~\citep{creager2021environment,ye2022ood}, graph invariant learning~(GIL) has recently emerged as a prominent solution for tackling its counterpart problem in graph data~\citep{li2022learning,fan2022debiasing,miao2022interpretable,wu2022discovering}. The fundamental assumption underlying GIL is that each graph sample can be divided into two distinct components, namely \textit{invariant subgraph} and \textit{environment subgraph}. The former exhibits deterministic and solid predictive relationships with the label of the graph sample, while the latter may show spurious correlations with the labels and can vary significantly in response to distribution shifts~\citep{yang2022learning,chen2024does}. By effectively separating invariant and environment information,  GIL-based approaches can learn invariant representations from the former and make reliable predictions. To achieve accurate separation, existing methods primarily focus on capturing and modeling the environmental subgraphs, employing carefully designed loss functions to minimize the correlations between the predicted environmental subgraphs and the labels~\citep{gui2024joint,piao2024improving}, or utilizing data augmentation strategies to simulate potential environments in wild data~\citep{wu2022handling,jia2024graph}.
\begin{figure}[t!]   

 \centering
 \subfigure[Diversity of environments.]{
   \includegraphics[width=0.21\textwidth]{1_intro/intro1.pdf}
   \label{subfig:intro1}
 } 
 \subfigure[Semantic cliff across classes.]{
   \includegraphics[width=0.21\textwidth]{1_intro/intro2.pdf}
   \label{subfig:intro2}
}
\vspace{-5mm}
\caption{Case examples of two challenges faced by graph out-of-dirstribution generalization}
\vspace{-8mm}
\label{fig:moti}
\end{figure}
Although GIL-based methods are theoretically viable, they underestimate the \textbf{difficulties in capturing environment information} in real-world graph data. These difficulties can be attributed to the \textit{diversity}, \textit{distinguishability}, and \textit{lack of labels} of practical graph environments. 
Specifically, the environments of graph data can exhibit substantial diversity in terms of sizes, shapes, and topological properties. Taking molecular graphs as an example (Fig.~\ref{subfig:intro1}), the invariant subgraph can be a specific functional group, while the environmental subgraphs may display varied patterns, such as different scaffolds, side chains, or bonding configurations that modify the overall structure~\citep{zhuang2023learning}. In this context, even with augmented or reorganized environments during training, GNN models struggle to identify all forms of environment subgraphs in real-world OOD samples. 
Moreover, unlike image data where environments can be clearly segmented at the pixel level, the structural boundaries between invariant and environmental subgraphs in graph data are often ambiguous (see the examples in Fig.~\ref{subfig:intro1}), which leads to poor distinguishability of environments. Moreover, unlike certain visual datasets~\citep{lin2022zin} where environment labels (such as background or image style) are available for model training, the environments in graph data are highly complex, making it difficult to obtain corresponding labels to aid in capturing environmental information. Given the above difficulties, most existing GIL-based approaches demonstrate suboptimal performance in identifying environmental information, particularly in complex graph data, as empirically demonstrated by~\citep{chen2024does}. Consequently, a natural question arises: \textbf{\textit{(RQ1) Can we consider a more feasible way to learn invariant representations on graphs without explicitly modeling the environment information?}}

In addition to the challenges posed by environment capturing, another critical obstacle, referred to as the \textbf{semantic cliff across different classes}~\citep{xia2024understanding}, also hinders current GIL-based approaches from making reliable decisions on OOD graph data. To be more specific, the semantic cliff issue refers to a situation where invariant subgraphs or representations from different classes share significant similarities, making them difficult to distinguish from one another~\citep{van2022exposing}.
For instance, as shown in Fig.~\ref{subfig:intro2}, invariant subgraphs (e.g., functional groups) across different molecular classes often share similar structural characteristics, with distinctions frequently limited to a single atom or bond. In such cases, the decision boundaries between invariant representations can become blurred, exacerbating the challenge of separating classes, particularly when the invariant and environment subgraphs are not distinctly identifiable. Nevertheless, the existing OOD generalization GNNs overemphasize the extraction of invariant information while neglecting the distinction between invariant subgraphs belonging to different classes, which may lead to their sub-optimal performance. Given this shortage, a natural follow-up question arises: \textbf{\textit{(RQ2) How can we develop a more robust OOD generalization approach that better discriminates between invariant representations across different classes?}}

To answer the above research questions, in this paper, we propose a novel \textbf{M}ulti-\textbf{P}rototype \textbf{H}yperspherical \textbf{I}nvariant \textbf{L}earning (\ourmethod for short) method. Building upon and enhancing the theoretical framework of GIL, \ourmethod propose a novel graph OOD generalization framework with two advanced features: 1)~\textbf{invariant learning in hyperspherical space}, which ensures the separability and informativeness of the learned invariant representations, and 2)~\textbf{class prototype as intermediate variable}, which eliminates the need for explicit environment modeling in invariant learning and enables flexible decision boundaries for prediction. 
More specifically, we derive a more practical invariant learning objective based on prototypical learning in hyperspherical space, incorporating two well-crafted loss terms. To address \textbf{\textit{(RQ1)}}, we design an \textit{invariant prototype matching loss} ($\mathcal{L}_{IPM}$) that ensures samples from the same class are assigned to the same class prototype in hyperspherical space. In this way, $\mathcal{L}_{IPM}$ can allow the model to extract robust invariant features across varying environments without explicitly modeling them. To answer \textbf{\textit{(RQ2)}}, we produce a \textit{prototype separation loss} ($\mathcal{L}_{PS}$) that pulls the prototypes belonging to the same class closer together while ensuring those from different classes remain dissimilar. In this way, $\mathcal{L}_{PS}$ enhances the class separability in the context of OOD generalization and mitigates the semantic cliff issue in graph data. Innovatively, we propose to assign multiple prototypes for each class, which ensures adaptable decision boundaries and greater tolerance to environmental changes. To sum up, the main contributions of this paper are as follows:

\begin{itemize}[leftmargin=*]
    \item \textbf{Framework.} Derived from the objective of GIL, we introduce a novel invariant learning framework that leverages hyperspherical space and prototypical learning, ensuring robust invariant representation learning while reducing the need for explicit graph environment modeling. 
    
    \item \textbf{Methodology.} Based on the new GIL framework, we develop a new graph OOD generalization method termed \ourmethod. \ourmethod incorporates two effective loss terms to enhance intra-class invariance and inter-class separability, with a multi-prototype mechanism to handle diverse environments.
    
    \item \textbf{Experiments.}  We conduct extensive experiments to validate the effectiveness of \ourmethod, and the results demonstrate its superior generalization ability compared to state-of-the-art methods across various types of distribution shifts.
\end{itemize}

% \begin{figure*}[h]
% \centering 
% \subfigure[Two molecular graphs with the same functional group but a different scaffold] { 
% \includegraphics[width=0.4\columnwidth]{1_intro/fig1.pdf} 
% }
% \subfigure[K] { 
% \includegraphics[width=0.4\columnwidth]{1_intro/fig2 (2).pdf} 
% }

% \caption{Left, Middle:} 
% \label{t-sne}
% \vspace{-1pt}
% \end{figure*}
% \begin{figure*}[t!] 
% \centering    
% \includegraphics[scale=0.39]{1_intro/sx_fig1(1).png}
% \caption{Upper: molecular graphs with the same functional group but different scaffolds. down:  molecular graphs with the different functional group which is too similar. }  
% \label{fig:intro} 
% \end{figure*}

==> 2_preliminary/pre_v1.tex <==
\subsection{notion and problem formulation}
OOD generalization in graph classification presents significant challenges due to varying distributions across different environments.  In this setting, we consider a pair of random variables: $G \in \mathcal{G}$, representing a graph instance, and $y \in \mathcal{Y}$, its corresponding label. The supervised training data is collected from multiple environments, denoted as $\varepsilon_{tr}$. Formally, the dataset can be expressed as $D = \{D^{e}\}_{e \in \varepsilon_{tr}}$, where $D^{e} =\{(\mathcal{G}^{e}_{i},\mathcal{Y}^{e}_{i})\}^{n^{e}}_{i=1}$  represents the data from environment $e$, and $n^e$ is the number of instances in environment $e$. Each pair $(\mathcal{G}^{e}_{i}, \mathcal{Y}^{e}_{i})$ is sampled independently from the joint distribution $P_{e}(\mathcal{G}, \mathcal{Y}) = P(\mathcal{G}, \mathcal{Y} | e)$.


% We focus on the OOD generalization for graph classification that involves a pair of random variables over instances $G \in \mathcal{G} $ and $y \in \mathcal{Y}$, where $G$ represents the graph and $\mY$ represents its corresponding label.  Generally, our supervised training dataset are collected from a set of training environments $\varepsilon_{tr}: D =\{D^{e} \}_{e \in \varepsilon_{tr}}$, where $D^{e} =\{(\mG^{e}_{i},\mY^{e}_{i})\}^{n^{e}}_{i=1}$ is the dataset from environment $e \in \varepsilon_{tr}$ and $n^{e}$ is the number of instances in environment $e$. Each $(\mG^{e}_{i},\mY^{e}_{i})$ is an i.i.d. draw from the joint distribution $P_{e}(\mG,\mY) = P(\mG,\mY | e)$.

Graph classification under OOD settings introduces additional complexities compared to traditional supervised tasks. This difficulty arises from the discrepancy between the training data distribution $P_{e_{tr}}(\mathcal{G}, \mathcal{Y})$ for environments $e_{tr} \in \varepsilon_{tr}$, and the testing data distribution $P_{e_{test}}(\mathcal{G}, \mathcal{Y})$ for unseen environments $e_{test} \in \varepsilon_{test}$. The goal of OOD generalization is to learn an optimal predictor $f: \mathcal{G} \rightarrow \mathcal{Y}$ that performs well across both training and unseen environments, $\varepsilon_{all} = \varepsilon_{tr} \cup \varepsilon_{test}$. This can be formalized as the following optimization problem: 
\begin{equation}
\label{eq: OOD_target} \min_{f \in \mathcal{F}} \max_{e \in \mathcal{E}_{\mathrm{all}}} \mathbb{E}_{(G^{e}, Y^{e}) \sim P_{e}}[\ell(f(G^e), Y^e)], 
\end{equation}
where $\mathcal{F}$ denotes the hypothesis space, and $\ell(\cdot,\cdot)$ represents the empirical risk function. However, the complexity of graph structures makes it challenging to define meaningful environments for OOD generalization.

% where $\mathcal{F}$ is hypothesis space and $\ell(\cdot,\cdot )$ is the empirical risk function. The definition of environment is natural and easily accessible in fields such as computer vision. However, it is challenging or even impossible for a graph $G=(A,X)$ with structure information $A$ and feature due to its  non-Euclidean complexity.


% \begin{figure}[htbp]
%     \centering
%     \subfigure[Covariate SCM{
%         \label{scm1} \includegraphics[width=0.3\textwidth,height=0.3\textwidth]{ICLR 2025 Template/scm1.png} % 替换 image_a 为你的图片文件名
%     }
%     \subfigure[FIIF SCM]{
%         \label{scm2} \includegraphics[width=0.3\textwidth,height=0.3\textwidth]{ICLR 2025 Template/scm2.png} % 替换 image_b 为你的图片文件名
%     }
%     \subfigure[PIIF SCM]{
%          \includegraphics[width=0.3\textwidth,height=0.3\textwidth]{ICLR 2025 Template/scm3.png} % 替换 image_d 为你的图片文件名
%     }
%     \caption{Three structural causal models (SCMs) on graph distribution shifts, each node denotes a variable, and each directional edge represents causation. Grey nodes are variables that can be directly observed, white nodes means variables that can't get accessed.}
%     \label{fig_scm}
% \end{figure}

\subsection{Invariant learning}
% We build upon the graph generation process proposed by Chen, which has been widely adopted in research on analyse OOD generalization. As illustrated in Figure \ref{fig_scm}, the causal feature $G_{c}$ and the spurious feature $G_s$ jointly control the generation of the observed input feature of the graph $G$. Environmental factors $e$ influence $G_s$, causing it to vary in different environments , while $G_c$ remains stable. The causal feature $Z$ directly controls the label $y$, maintaining a stable relationship with it. In OOD scenarios, distribution shifts typically correspond to changes in environmental factors $e$ but with a  stable $G_c$. Moreover, the generation of $G_s$ may be influenced by the labels $y$ or the causal feature $G_c$, as depicted in Figures 1 (b) and 1(c), respectively.

Invariant learning focuses on capturing representations that remain consistent across different environments, aiming to ensure that the learned representation $z_{inv}$ maintains a stable relationship with the label $y$. Specifically, for graph OOD generalization, our goal is to learn an invariant GNN, $f:= f_{c} \circ g$, where $g: \mathcal{G} \rightarrow z_{inv}$ is an encoder that extracts the invariant representation from the input graph $G$, and $f_{c}: z_{inv} \rightarrow \mathcal{Y}$ is a classifier that predicts the label $y$ based on $z_{inv}$. From this perspective, the optimization objective of OOD generalization, as stated in Eq.\ref{eq: OOD_target}, can be reformulated as: 
\begin{equation}
\label{eq: causal} \max_{f_{c}, g} I(z_{inv}; y), \text{ s.t. } z_{inv} \perp e,\forall e \in \mathcal{E}_{tr}, z_{inv} = g(G). 
\end{equation}
This objective ensures that $z_{inv}$ remains independent of the environment $e$, focusing solely on the most relevant information for predicting $y$. While invariant learning offers a promising approach, it faces limitations in graph data, particularly due to the "semantic cliff." Small changes in a graph’s structure can lead to large shifts in labels, making the invariant representation of different class are not well-separable. This sensitivity highlights the inherent limitations of applying invariant learning to graphs.


% Invariant learning is primarily grounded in the data generation process shown in Figure 1, with the goal of enabling the model to learn the representation $z_{inv}$, which remains invariant across environments and exhibits the most stable correlation with the label $y$, treating it as the representation of  $G_{c}$. Specifically, for graph OOD generalization, our aim is to learn an invariant GNN $f:= f_{c} \circ 
%  h$, which is composed of a encoder $h : \mathcal{G} \rightarrow z_{inv}$ that extract invariant representation from the input graph $G$, and a classifier $f_{c} : z_{inv} \rightarrow \mathcal{Y}$ that predicts the label $y$ according to the $z_{inv}$. From tis prospective, the optimization objective of OOD generalization in Eq. (\ref{OOD_target}) can be reformulated as follows:
%  \begin{equation}\label{eq_causal}
%  \max_{f_{c}, h} I(z_{inv}; y), \text{ s.t. } z_{inv} \perp e,\forall e \in \mathcal{E}_{tr}, z_{inv} = h(G).
%  \end{equation}
%  This object ensures that $z_{inv}$ remains independent of the environment $E$, providing only the most relevant information about 
% $y$ under an additional constraint. However, identifying the precise environment of a graph proves to be challenging, even not infeasible, which presents a significant obstacle for achieving OOD generalization in graphs through invariant learning.
%\begin{equation}\label{eq_ib}
 %   \underset{\mZ}{\min} -I(\mY;\mZ)+\beta I(\mZ;\mX)
%\end{equation}
%where $I(\cdot;\cdot)$ is the mutual information between two variable and $\beta$ is the Lagrangian parameter to control the trade-off between the two terms. From the perspective of invariant learning, the Information Bottleneck (IB) approach can be viewed as an effective method for extracting features $z_{inv}=z$ from input $x$ that are invariant to the environment. This is because the first term of the Eq. (\ref{eq_ib}) ensures that $z$ retains the most relevant information for predicting the target $Y$, while the second term aim to compress the mutual information of $Z$ and $X$  to make $Z$ ignores irrelevant part of X with respect to the target $Y$. Thus the representation $Z$ which satisfy IB is more robust to noise and distribution shift and it has been proven to be an effective solution to solve the OOD generalization problem by several recent studies.
\subsection{graph hyperspherical embedding}
Hyperspherical embeddings enhance the discriminative ability and generalization of the model by mapping feature vectors onto a unit sphere. For a input graph $G$, its vector representation $z$ are encoded by a GNNs and then projected into a lower-dimensional hyperspherical space, followed by normalization to ensure that the projected vector $\hat{z}$ lies on the unit hypersphere.
% with $\hat{z} = MLP(z)$ and $\hat{z} = \hat{z} / \| \hat{z}\|_{2}$.
These hyperspherical embeddings $\hat{z}$ are modeled using the von Mises-Fisher (vMF) distribution, where the probability density for a unit vector in class $c$ is given by:
\begin{equation}
\label{eq: vMF} p(\hat{z}; \mu_c, \kappa ) = Z_d(\kappa) \exp(\kappa \mu_c^\top \hat{z}), 
\end{equation} 
where ${\mu}_c$ denotes the prototype of class $c$ with the unit norm and can also be treated as the mean direction of the class $c$, and $\kappa$ controls the concentration of samples around $\boldsymbol{\mu}_c$.
The term $Z_d(\kappa)$ serves as the normalization factor for the distribution. Given the probability model in Eq.(\ref{eq: vMF}), an embedding $\hat{\vz}_{i}$ is assigned to class $c$ with the following probability:
\begin{equation} \label{eq: prototpye_1}
    \begin{aligned}
p\left(y = c \mid \hat{z}; \{\kappa, \mu_{i}\}_{i = 1}^{C}\right) = \frac{Z_{d}(\kappa) \exp \left(\kappa \mu_{c}^{\top} \hat{z}\right)}{\sum_{i = 1}^{C} Z_{d}(\kappa) \exp \left(\kappa \mu_{i}^{\top} \hat{z}\right)} = \frac{\exp \left(\mu_{c}^{\top} \hat{z} / \tau\right)}{\sum_{i = 1}^{C} \exp \left(\mu_{i}^{\top} \hat{z} / \tau\right)},
    \end{aligned}
\end{equation}
where $\tau = 1/\kappa$ is a temperature parameter. While the hyperspherical embedding is naturally more separable and classifier friendly, ensuring its environmental robustness is critical for achieving effective OOD generalization in graph learning. The compatibility of this approach with invariant learning is particularly important, as the latter approach is guaranteed to learn a stable, environment-invariant hyperspherical representation. 


% Formulating the embedding space with a hypersphere model has been shown to be beneficial to obtain a more discriminative and well generalizated representation. We consider a deep neural network based encoder $h_{\theta} : \mathcal{X} \rightarrow \mathbb{R}^{d}$ that extract the feature embedding $z \in \mathbb{R}^{d}$ from the input $X \in \mathcal{X}$ with $z = h(x)$. A projector $g_{\phi} : \mathbb{R}^{d} \rightarrow \mathbb{R}^{\hat{d}}$ with normalization is utilized  to project the embedding $z$ from the original high-dimensional space to a low-dimensional space and obtain the hyperspherical embedding $\hat{z}$ via  $\hat{z} = g_{\phi}(z)$ and $\hat{z} = \hat{z} / \| \hat{z}\|_{2}$. The hyperspherical  embeddings $\hat{z}$ lying on the unit sphere ($\|\hat{z}\|^2 = 1$) can be naturally modeled by the von Mises-Fisher (vMF) distribution. The probability density for a unit vector $\hat{z} \in \mathbb{R}^{\hat{d}}$ in class $c$ is defined as :
% \begin{equation}\label{vMF}
%     p(\hat{\vz}; \boldsymbol{\mu}_c, \kappa )=Z_d(\kappa)\exp(\kappa\boldsymbol{\mu}_c^\top\hat{\vz}),
% \end{equation}

% where $\boldsymbol{\mu}_c$ denotes the prototype with unit norm and can also be treat as the mean direction of the class $c$ with $\boldsymbol{\mu}_c = \frac{1}{K} \sum \displaystyle_{k}\hat{\vz}_{k}, \vy_{k}=c$,  $\kappa$ represents the tightness around the $\boldsymbol{\mu}_c$ and $Z_d(\kappa)$ denotes the normalization factor. 

% Given the probability model in Eq.(\ref{vMF}), an embedding $\hat{\vz}_{i}$ is assigned to class $c$ with the following probability:
% \begin{equation} \label{prototpye_1}
%     \begin{aligned}
% p\left(y = c \mid \mathbf{z} ;\left\{\kappa, \boldsymbol{\mu}_{j}\right\}_{j = 1}^{C}\right)  = \frac{Z_{d}(\kappa) \exp \left(\kappa \boldsymbol{\mu}_{c}^{\top} \mathbf{z}\right)}{\sum_{j = 1}^{C} Z_{d}(\kappa) \exp \left(\kappa \boldsymbol{\mu}_{j}^{\top} \mathbf{z}\right)} 
%  = \frac{\exp \left(\boldsymbol{\mu}_{c}^{\top} \mathbf{z} / \tau\right)}{\sum_{j = 1}^{C} \exp \left(\boldsymbol{\mu}_{j}^{\top} \mathbf{z} / \tau\right)},
%     \end{aligned}
% \end{equation}
% where $\tau = 1/\kappa$ is a temperature parameter. Classification based on the distance to prototypes within hyperspherical embedding spaces has been widely adopted in OOD detection and has been practiced in OOD generalization. However, this approach has yet to gain significant traction within the graph learning community. Moreover, existing methods frequently overlook the robustness of the learned prototypes, that is, we hope that it is also invariant across environments to ensure that the out-of-distribution samples are matched to the correct prototype during classification.
%但我们需要跨环境不变的损失
% \section{motivation}
% Our work is motivated by maximizing inter-class invariance and inter-class separation without context dependence to ensure that the learned representations generalize to out-of-distribution environments while still being correctly classified by the model. This is inspired by the theoretical definition proposed by Ye et al, which shows that the error bound of OOD generalization is related to the \textit{Variation} and \textit{Informativeness} of the representation. The formal definitions are given as follows.

% \begin{definition}(Variation)\label{def_1}
% \textit{The variation of representation $\phi$ across a domain set $\mathcal{E}$ is}
% \begin{equation}
% \mathcal{V}(\phi, \mathcal{E}) = \max_{y \in \mathcal{Y}} \sup_{e, e' \in \mathcal{E}} \rho\left(\mathbb{P}(\phi^e | y), \mathbb{P}(\phi^{e'} | y)\right),
% \end{equation}
% \end{definition}

% \textit{where $\rho(\mathbb{P}, \mathbb{Q})$ is a symmetric distance (e.g., Wasserstein distance, total variation) between two distributions, and $\mathbb{P}(\phi^e | y)$ denotes the class-conditional distribution for features of samples in environment $e$. A feature $\phi$ is $\epsilon$-invariant across $\mathcal{E}$, if $\epsilon \geq \mathcal{V}(\phi, \mathcal{E})$.}
% \begin{definition}(Informativeness) 
% \textit{The informativeness of representation $\phi$ across a domain set $\mathcal{E}$ is}  
% \begin{equation}
% I_(\phi, \mathcal{E}) = \frac{1}{K(K-1)} \sum_{\substack{y \neq y' \\ y, y' \in \mathcal{Y}}} \min_{e \in \mathcal{E}} \rho\left(\mathbb{P}(\phi^e | y), \mathbb{P}(\phi^e | y')\right).
% \end{equation}
% \textit{A feature $\phi$ is $\delta$-informativeness across $\mathcal{E}$, if $\delta \leq \mathcal{V}(\phi, \mathcal{E})$.}
% \end{definition}
% Overall, \textit{Variation} measures whether the learned representations of the same class remain invariant across environments, while \textit{Informativeness} describes the distinguishability of these representations with respect to class. Furthermore, Ye et al. extended these definitions by providing an error bound for OOD generalization, theoretically proving that if a learner trained on in-distribution data can simultaneously minimize Variation and maximize Informativeness, it can generalize to the out-of-distribution.

% It is worth noting that although Variation and Informativeness are theoretically clear and reasonable, directly using them as optimization objectives to improve the generalization ability of GNNs is challenging. First, as mentioned in previous sections, it is difficult to obtain environment information in graph data. Second, the semantic cliff of graphs makes it more challenging to ensure that invariant features also exhibit high Informativeness. In the following sections, we will introduce how we leverage two practical loss functions to learn representations that achieve low \textit{Variation} and high \textit{Informativeness}.
% \subsection{main optimization objective }
% First, we give the overall optimization objective of the model, it can be formulated as follows:
% \begin{equation}
%     \mathcal{L}= \mathcal{L}_{intra-inv} + \mathcal{L}_{inter-sep} +\mathcal{L}_{cls},
% \end{equation}
% Overall, intra-class invariance is achieved by minimizing $\mathcal{L}_{intra-inv}$, while minimizing $\mathcal{L}_{inter-sep}$ is equivalent to maximizing inter-class separability. Finally, $\mathcal{L}_{cls}$ ensures the learned representation remains highly relevant to the label. All these operations are performed in hyperspherical space and do not require environmental information.
% \subsection{intra class invariance without $\mathcal{E}$}
% Now we introduce the loss function $\mathcal{L}_{intra-inv}$ that guarantees the learned representation is invariant across environments $\mathcal{E}$ without relying on detail environmental labels. It can be formulated as follows:
% \begin{equation}
%     \mathcal{L}_{intra-inv}= - \frac{1}{C}\sum_{y_c}^{C} \sum_{i=1}^{|y^c|} \log \frac{\underset{c=\hat{c} = y_c}{\sum}\exp \left( {(z_i^c)^\top (z_j^{\hat{c}}) }/{\tau} \right)}{\underset{c=\hat{c}=y_c}{\sum}\exp \left( {(z_i^c)^\top (z_j^{\hat{c}}) }/{\tau} \right)+\underset{c=y_{c},\hat{c} \neq y_c}{\sum}\exp \left( {(z_i^c)^\top (z_j^{\hat{c}}) }/{\tau} \right)} ,
% \end{equation}
% Intuitively, minimizing $\mathcal{L}_{intra-inv}$ corresponds to clustering the invariant features of samples from the same class as tightly as possible within the subspace of the hypersphere corresponding to that class, while ensuring a clear boundary between this subspace and those of other classes. This clustering-like approach does not require environmental information, as it guarantees that invariant representations of the same class remain close, regardless of the environment, thereby ensuring intra-class invariance.

% Next we theoretically prove the effectiveness of this loss. Frist, to align the objective in Definition \ref{def_1} with the cause-effect-based graph generation process shown in Figure 1, we present the following proposition to demonstrate that optimizing Variation is equivalent to satisfying the condition in Eq. (\ref{eq_causal}), meaning that the invariant features are independent of the environment.
% \begin{proposition}
% Minimizing Variation in Definition \ref{def_1} is equivalent to learning a $z_{inv}$ satisfying $z_{inv} \perp E$
% \end{proposition}
% This proposition further illustrates that minimizing intra-class variability guarantees the learned invariant representation and environment independence, and next we will give a theorem proving the relationship between loss function and variation.
% \begin{theorem}
%     if $\max_{y \in \mathcal{Y}}\min_{c=\hat{c}=y}\exp ( (z_i^c)^\top (z_j^{\hat{c}})) = \epsilon $, then we can have $f(\epsilon)  \geq \mathcal{V}(\phi, \mathcal{E})$ and say $z$ is $f(\epsilon)$-invariant across $\mathcal{E}$, where $f$ is  a monotonically increasing function depending on how the distribution distance is calculated, $\rho$. 
% \end{theorem}
% The above theorem theoretically proves that when we minimize the distance between invariant representations of the same category by minimizing the loss function, intra-class invariance can be guaranteed without the help of the environment
% \subsection{inter class separability with prototype ${\mu}^c$}
% We know that optimizing $\mathcal{L}_{intra-inv}$ can yield invariant features, but relying solely on these features is insufficient to achieve robust OOD generalization. It is crucial to ensure that the learned invariant features are class-discriminative, as we do not want the model to capture information unrelated to the label $y$, such as fixed noise. To address this, we propose maximizing inter-class separability to ensure correct classification, which is formally defined as follows:
% \begin{equation}
%     \mathcal{L}_{intra-inv} = \frac{1}{C} \sum_{i=1}^{C} \log \left( \frac{1}{C-1} \sum_{\substack{j \neq i,j \in \mathcal{Y}}} \exp \left( {\mu_i^\top \mu_j}/{\tau} \right) \right),
% \end{equation}
% The effectiveness of optimizing $\mathcal{L}_{intra-inv}$ lies in the fact that our classification is distance-based with respect to prototypes, so increasing the distance between different prototypes helps to enhance separability. Note that in hyperspherical space, prototypes can often be viewed as the center of a class.We also ensure that the learned invariant features match the correct prototype as much as possible by optimizing the classification loss $L_{cls}$ (cross entropy). Thus, ensuring the separability of the prototypes guarantees that the invariant features are also class-separable.

% First of all, we propose the following proposition that guarantees to minimize $L_{cls}$ such that the learned invariant representation is the most relevant to the label.
% \begin{proposition}
% Minimizing $L_{cls}$  is equivalent to learning a $z_{inv}$ that can maximum the $I(z_{inv};y)$.
% \end{proposition}
% However, when labels with similar semantics or invariant subgraphs are fragile, only minimizing $L_{cls}$cannot satisfy the inter-class separability. We propose the following proof to theoretically prove the feasibility of $L_{intra-inv}$.
% \begin{theorem}
%     if $\sum_{y \in \mathcal{Y}}\max{c=y}\exp ( (z_i^c)^\top (\mu^{{c}})) = \epsilon $ and $\sum_{y \in \mathcal{Y}}\min_{c=y, \hat{c}\neq y}\exp ( (z_i^c)^\top (z_j^{\hat{c}})) = \gamma$, then we can have $f(\gamma-2\epsilon)  \leq \mathcal{V}(\phi, \mathcal{E})$ and say $z$ is $f(\gamma-2\epsilon)$-informativeness across $\mathcal{E}$, where $f$ is  a monotonically increasing function depending on how the distribution distance is calculated, $\rho$. 
% \end{theorem}
% The above theorem further ensures that the learned invariant features are inter-class separable by increasing the distance between class prototypes in the hyperspherical space.

==> 3_method/method_v1.tex <==
 \begin{figure*}[t!]    % 常规操作\begin{figure}开头说明插入图片
					% 后面跟着的[htbp]是图片在文档中放置的位置，也称为浮动体的位置，关于这个我们后面的文章会聊聊，现在不管，照写就是了
					\centering    
% 前面说过，图片放置在中间
	\label{fig:subfig5}\includegraphics[scale=0.39]{framework.jpg}
				
					
					\caption{During the training phase, we map the input graph to invariant features using a GNN-based extractor and project them into the hyperspherical space. The invariance of these features with respect to the environment is enforced by minimizing $\mathcal{L}_{\text{inv}}$, while the maximum separability of the categories within the hyperspherical space is ensured by minimizing $\mathcal{L}_{\text{sep}}$}    % 整个图片的说明，注释写在{}内
					\label{framework}            % 整个图片的标签编号，注意这里跟子图是一样的道理，标签不能重复 
				\end{figure*}

As previously mentioned in Eq.(\ref{eq: causal}), the OOD generalization objective seeks to maximize the mutual information between the invariant representation $z_{inv}$ and the label $y$, while ensuring that $z_{inv}$ remains independent of the environment $e$. However, directly optimizing this objective with strict constraints is challenging, especially in the context of graph data where defining and partitioning environments is inherently difficult. Graph structures do not have clear environmental boundaries, making it hard to enforce environment-specific constraints. To make the optimization more tractable, we relax the independence constraint and introduce a soft-constrained formulation: 
\begin{equation}
\label{eq: IB}
   \underset{z_{inv}}{\min} -I(y; z_{inv})+\beta I(z_{inv};e),
\end{equation}
where $e$ represents the environment to which the current graph belongs, but it cannot be directly observed or obtained. The parameter $\beta$ controls the trade-off between the predictive power of $z_{inv}$ and its independence from the environment $e$. This soft constraint allows for a more flexible optimization that still maintains the desired invariance properties in graph-based OOD generalization. Rather than relying on the explicit definition of the environment $e$, which is inherently difficult in graph data, we adopt a more flexible approach by using  prototypes in the hyperspherical space as implicit representations of environmental variations. This enables us to achieve the desired invariance in a more practical manner.


\textbf{Definition 1} (Prototype as Environment Variants). \label{def_1} 
\textit{For each class \( c \), we define its prototype denoted as \( \mu_{c} \). A graph $G_i$ will be classified as the class $i$ only if its hyperspherical representation \( \hat{z}_i \) has the greatest similarity with prototype \( \mu_{i} \). If  two  hyperspherical representations with different classes \( \hat{z}_i \in \mathcal{Y}_a \) and \( \hat{z}_j \in \mathcal{Y}_b \) are mistakenly assigned to the same prototype, i.e.,
\[
\mathrm{argmax}_{i} \, \mathrm{sim}(\hat{z}_i, \mu_{i}) = \mathrm{argmax}_{i} \, \mathrm{sim}(\hat{z}_j, \mu_{i})
\]
this misclassification suggests that the hyperspherical representations \( \hat{z} \) are more influenced by the environment \( e \) than by the actual class labels \( y \). Therefore, we can infer that this misclassification likely arises from the two graphs being in the same environment.}%Therefore, by increasing the number of prototypes, these prototypes can implicitly represent the environmental variations, eliminating the need to explicitly define or separate the environment \( e \).}

Given the introduction of prototypes as implicit variants of environment $e$, we now perform invariant learning in hyperspherical space and reformulate the optimization objective: 
\begin{equation}\label{eq: target2}
   \underset{\hat{z}_{inv}}{\min} \underbrace{-I(y ; \hat{z}_{inv}|\mu_{y}) }_{\mathcal{L}_{\mathrm{cls}}}\underbrace{-I(y ; \mu_{y}|\hat{z}_{inv}) }_{\mathcal{L}_{\mathrm{PS}}}+\underbrace{\beta I\left(\hat{z}_{inv};e|\mu_{y}\right)}_{\mathcal{L}_{\mathrm{IPM}}}.
\end{equation}
where $\hat{z}_{inv}$ represents the hyperspherical invariant representation. By using prototypes to represent environmental variations, we avoid the need for explicitly defining or labeling the environment. In addition, we guarantee the separability of the hyperspherical representation by increasing the distance between prototypes of different classes. Next, we will analyze each component of Eq.(\ref{eq: target2}) to provide a detailed understanding of its meaning. Additionally, the overall framework is illustrated in Figure 1, and the detailed pseudocode for the training process can be found in Appendix 1.

\subsection{hyperspherical invariant representation  extraction model}\label{invariant_model}
The goal of invariant learning is to extract features that are associated only with the label and remain invariant across environments. In the case of graph data, this usually means identifying an invariant subgraph. However, extracting flexible and variable subgraphs from complex, non-Euclidean structures can be time-consuming and often infeasible. Instead, we extract invariant representations in the latent space, which is both efficient and consistent with our loss function in Eq. (\ref{eq: target2}).

We utilize two GNNs: one to encode the input graph $G$ into the latent space, producing the node representation  $\mathbf{H}$, and the other to compute the separation score $S$ for the invariant features: 
\begin{equation}
    \mathbf{H} = \mathrm{GNN}_{I}(G) \in \mathbb{R}^{|\mathcal{V}| \times d}, \mathbf{S} = \sigma(\mathrm{GNN}_{S}(G)) \in \mathbb{R}^{|\mathcal{V}| \times d},
\end{equation}
$\mathrm{GNN}_{I}$ encodes the input graph and $\mathrm{GNN}_{S}$ computes the separation score. $|\mathcal{V}|$ is the number of nodes in the graph $G$, $d$ is the latent space dimension, and $\sigma(\cdot)$ is the Sigmoid function to constrain $\mathbf{S}$ falls into the range of $(0,1)$. The invariant representation $\mathbf{z}_{inv}$ is  obtained through the following operation:
\begin{equation}
    \mathbf{z}_{inv} = \mathrm{READOUT}(\mathbf{H} \odot \mathbf{S}) \in \mathbb{R}^{d},
\end{equation}
where $\odot$ is the element-wise product and $\mathrm{READOUT}$ is an aggregation function (e.g., $\mathrm{mean}$) to generate a graph-level representation. Existing graph invariant learning methods optimize the objective in Eq. (\ref{eq: IB}) using $z_{inv}$, but this often relies on explicit environment information and fails to ensure sufficient class separability. 
Our approach optimizes a more achievable objective Eq. (\ref{eq: target2}) by computing hyperspherical invariant representations $\hat{z}_{inv}$. It can be formulated as follows:
\begin{equation}
\label{eq: hype_rinv}
    \hat{z}_{inv} = \mathrm{Poj}(z_{inv}), \hat{z}_{inv} = \hat{z}_{inv} / \| \hat{z}_{inv}\|_{2}
\end{equation}
where $\mathrm{Poj}$ is a projector, such as an $\mathrm{MLP}$, that maps the representation to a lower-dimensional space.  This method establishes a novel framework by integrating invariant learning with hyperspherical embeddings, laying the groundwork for the introduction of prototypes. By leveraging hyperspherical space, the model mitigates the need for explicit environmental labels and enhances the separability of class representations. Hyperspherical invariant representation strengthens OOD generalization and sets the foundation for incorporating prototypes to refine the learned representations further.

\subsection{Multi prototypes based hypersphere model} 
In the previous section, we established the groundwork for using hyperspherical embeddings to enhance representation separability. While traditional prototype-based models map input directly into hyperspherical space and rely on a single prototype for each class, this approach can result in non-compact representations and unclear decision boundaries. A single prototype often overfits easy-to-classify samples while failing to account for harder cases. To address these limitations, we extend the hyperspherical space by introducing multiple prototypes for each class, allowing the model to better capture the full complexity of the data. This multi-prototype approach ensures that the classification decision space is more adaptable and comprehensive, leading to more accurate coverage of all sample types.

\subsubsection{prototype updating}
To implement this multi-prototype approach effectively, it is essential to maintain up-to-date prototypes for each class throughout the training process. The following section describes the prototype updating mechanism that ensures the prototypes remain representative of their respective classes. 

Specifically, we assign $K$ prototypes for each class $c$ with $\boldsymbol{\mu}^{c} = \{ \boldsymbol{\mu}^{c}_{k}\}^{K}_{k=1}$
 and each prototype can be initialized as follows:
\begin{equation} \label{init}
 \quad \mu^{c}_{k} \sim \mathcal{N}(\textbf{0}, \textbf{I}), \quad 
\end{equation}
where $\mathcal{N}(\textbf{0}, \textbf{I})$ represents a standard multivariate Gaussian distribution, with mean vector $\textbf{0}$ and identity covariance matrix $\textbf{I}$. To ensure that the prototypes remain representative of the majority of samples in their respective classes, we adopt the exponential moving average (EMA) technique, which updates the prototypes asynchronously.

After obtaining the hyperspherical invariant representation $\hat{z}_{inv}$, the corresponding class prototype is updated before applying gradient descent to Eq.(\ref{eq: target2}) to adjust the model parameters. This approach prevents the prototype values from fluctuating too much during training, avoiding suboptimal solutions. The update rule for a batch of $B$ samples is given by:
\begin{equation} \label{eq: update_prototype}
    \boldsymbol{\mu}_k^c := \text{Normalize}\left( \alpha \boldsymbol{\mu}_k^c + (1 - \alpha) \sum_{i=1}^{B} \mathbbm{1}(y_i = c) w_{i,k}^c \hat{\vz}^i_{inv} \right), 
\end{equation}
where $\alpha$ is the EMA update rate, $w_{i,k}^c$ is the weight of sample $i$ for prototype $k$ in class $c$, and $\mathbbm{1}(y_i = c)$ is an indicator function that ensures the update applies only to samples of class $c$.  After each update, the prototype is normalized to maintain its unit norm, ensuring it remains on the hypersphere. The $\text{Normalize}$ function ensures that the prototypes are re-normalized to the unit sphere, allowing distance calculations to take place in the same space as $\hat{\vz}^i_{inv}$. Each representation $\hat{\vz}^i_{inv}$ is associated with multiple prototypes, weighted by the assigned weight vector$w_{i}^c \in \mathbb{R}^{K}$. By updating the prototypes using $\hat{z}_{inv}$, we ensure that the prototypes remain robust to environmental variations. This provides a clear advantage over traditional hyperspherical spaces, making our method particularly well-suited for OOD generalization tasks. 


\subsubsection{weight calculation and pruning}
Once the prototypes have been updated to reflect their respective class centers, it becomes critical to assign appropriate weights to ensure that each sample is matched with the most relevant prototype. In our multi-prototype hypersphere model, we address this through an Attention-based Matching mechanism. This approach computes the attention score between each sample and its corresponding class prototypes to determine the matching probability.
We first compute the attention scores as follows:
\begin{align}\label{eq: att}
    Q = \hat{\vz}_{inv}\mW^{Q}, K = \boldsymbol{\mu}^c\mW^{K}, \vw^{c} = \mathrm{softmax}(\frac{QK^\top}{\sqrt{d'}}),
\end{align}
where $\mW^{Q}, \mW^{K} \in \mathbb{R}^{d \times {d'}}$ are the learnable weight matrices for the samples and the prototypes, respectively. $d'$ is the dimension of the projected space.  The attention mechanism ensures that the prototype $\boldsymbol{\mu}^c$ most similar to $\hat{\vz}_{inv}$ receives the highest weight, which improves classification accuracy and helps the prototype remain aligned with its class center.

However, assigning weights to all prototypes within a class can lead to excessive similarity between prototypes, especially for difficult samples. This could blur decision boundaries and reduce the model's ability to correctly classify hard-to-distinguish samples.

To address this, we apply a \textbf{top-$k$ pruning} strategy, which keeps only the $k$-most relevant prototypes for each sample. The top-$k$ weights are retained, and the rest are pruned as follows:
\begin{equation}
    w_{i,k}^c = \mathbbm{1}[w_{i,k}^c>\beta]\ast w_{i,k}^c, 
\end{equation}
where $\beta$ is the threshold corresponding to the $k$-th largest weight, and $\mathbbm{1}[_{i,k}^c>\beta]$ is an indicator function that retains only the weights for the top-$k$ prototypes. This pruning mechanism ensures that the prototypes remain distinct and that the decision space for each class is well-defined, allowing for improved classification performance. By applying this attention-based weight calculation and top-$k$ pruning, the model ensures a more accurate and robust matching of samples to prototypes, enhancing classification, especially in OOD scenarios.

\subsection{Optimization Objectives for MPHIL}

\subsubsection{Invariant prototype matching loss $\mathcal{L}_{\mathrm{IPM}}$}
The challenge of disentangling invariant features from environmental variations lies at the heart of OOD generalization.   In our formulation, the misalignment of a sample with an incorrect prototype can be seen as a signal of environmental interference, while successful alignment with the correct prototype reflects the capture of stable, invariant features. The $\mathcal{L}_{\mathrm{IPM}}$ operates by reinforcing the proximity of samples to their invariant representations and penalizing the influence of environmental factors, implicitly captured through incorrect prototype associations.
The loss function is expressed as follows:
\begin{align}
   \mathcal{L}_{\mathrm{IPM}} = - \frac{1}{B} \sum_{i=1}^{B} \log \frac{\sum_{c=y_i} \exp \left( \hat{z}_i^\top \boldsymbol{\mu}^c / \tau \right)}{\sum_{c=y_i} \exp \left( \hat{z}_i^\top \boldsymbol{\mu}^c / \tau \right) + \sum_{\hat{c} \neq y_i} \exp \left( \hat{z}_i^\top \boldsymbol{\mu}^{\hat{c}} / \tau \right)},
\end{align}
where $B$ represents the batch size, with $i$ indexing each sample in the batch. $\hat{z}_i$ represents the hyperspherical invariant representation, $\boldsymbol{\mu}^c$ is the correct class prototype, and $\boldsymbol{\mu}^{\hat{c}}$ denotes the prototypes of the incorrect classes $\hat{c} \neq y_i$. $\tau$ is a temperature factor. This formulation reflects the dual objective of pulling samples towards their class-invariant prototypes while ensuring that the influence of prototypes associated with environmental shifts is minimized. The numerator reinforces the similarity between the sample’s invariant representation and its correct prototype, while the denominator introduces competition between correct and incorrect prototypes, implicitly modeling the influence of environmental noise.

\subsubsection{Prototype Separation Loss $\mathcal{L}_{\text{PS}}$}
In hyperspherical space, all invariant $\hat{z}$ representations are compactly clustered around their respective class prototypes. To ensure inter-class separability, prototypes of different classes must be distinguishable.  The Prototype Separation Loss $\mathcal{L}_{\text{PS}}$  is designed to enforce this by maximizing the separation between prototypes of different classes while encouraging the similarity of prototypes within the same class. The loss function is defined as:
\begin{equation}
    \mathcal{L}_{\text{PS}} = -\frac{1}{CK} \sum_{c=1}^{C} \sum_{k=1}^{K} \log \frac{\sum_{i = 1}^{K} \mathbb{I}(i \neq k) \exp \left( {(\mathbf{\mu}_k^c)^\top \mathbf{\mu}_{i}^c}/{\tau} \right)}{\sum_{c' = 1}^{C} \sum_{j = 1}^{K} \mathbb{I}(c' \neq c) \exp \left( {(\mathbf{\mu}_k^c)^\top \mathbf{\mu}_{j}^{c'}}/{\tau} \right)},
\end{equation}
where $C$ represents the total number of classes, and $K$ denotes the number of prototypes assigned to each class. The prototypes $\mathbf{\mu}_k^c$ and $\mathbf{\mu}_i^c$ correspond to different prototypes within the same class $c$, while
$\mathbf{\mu}_k^c$ and $\mathbf{\mu}_j^{c'}$ represent prototypes from different classes.  The indicator function
$\mathbf{\mu}_k^c$ and $\mathbf{\mu}_j^{c'}$ represent prototypes from different classes.  The indicator function ensures that the comparisons are made between distinct prototypes, enhancing intra-class similarity and inter-class separation.


\subsubsection{prediction}
Given the complexity of real-world graph data, a single prototype per class often fails to capture the full diversity of features, especially in cases where graph structures are highly variable. Therefore, we modify Eq. (\ref{eq: prototpye_1}) to accommodate a multi-prototype setting. This multi-prototype strategy allows the invariant representations $\hat{\vz}_{inv}$ to learn more robust features, enhancing the model's ability to handle difficult-to-classify samples and reducing the likelihood of misclassification due to environmental variations.

In this setup, each class is represented by multiple prototypes, and the classification decision is made based on the maximum similarity between the invariant representation $\hat{\vz}_{inv}$ and the set of prototypes $\boldsymbol{\mu}_{k}^{c}$ associated with each class. The prediction probability is defined as:
\begin{equation}\label{classify}
   p(y = c | \hat{\vz}_{inv}; \{ \mathbf{w}^j, \boldsymbol{\mu}^c, \kappa \}_{j=1}^C) = 
\frac{\underset {k=1,\dots,K}{\max} (w_{k}^c \exp \left(  {\boldsymbol{\mu}_k^c}^\top \hat{\vz}_{inv} / \tau \right))}
{\sum_{j=1}^{C} \underset {{k'}=1,\dots,K}{\max} (w_{k'}^j \exp \left(  {\boldsymbol{\mu}_{k'}^j}^\top \hat{\vz}_{inv} / \tau \right))}.
\end{equation}

During training, this classification probability is used to compute the cross-entropy loss ${\mathcal{L}_{\mathrm{cls}}}$ which is defined as:
\begin{equation}
    \mathcal{L}_{\text{cls}} = \text{Cross-entropy}(y, \mathrm{argmax}_{c} p(y = c \mid \hat{\vz}_{inv}; \{ \boldsymbol{\mu}_k^c \}_{j=1}^C)).
\end{equation}

In this chapter, we introduced the Multi-Prototype Hyperspherical Invariant Learning (MPHIL) framework, which leverages hyperspherical embeddings and a multi-prototype strategy to improve OOD generalization in graph data. By utilizing prototypes as implicit representations of environmental variations and optimizing a relaxed objective, our method effectively captures invariant features and enhances class separability. The training procedure, including prototype updating and weight pruning, is detailed in the pseudocode provided in Appendix A.

==> 4_exp/exp_v1.tex <==
In this section, we verify the effectiveness of our methods by conducting comprehensive experiments on two graph OOD benchmarks. 
\subsection{Experiments setup}
\textbf{Datasets.} We utilize two real-world benchmarks with various distribution shifts to evaluate our method. GOOD is a comprehensive graph OOD benchmark, and we selected three datasets: (1) GOOD-HIV, a molecular graph dataset predicting HIV inhibition; (2) GOOD-CMNIST, containing graphs transformed from MNIST using superpixel techniques; and (3) GOOD-Motif, a synthetic dataset where graph motifs determine the label. Additionally, DrugOOD is designed for AI-driven drug discovery with three types of distribution shifts: scaffold, size, and assay, applied to six molecular datasets for predicting drug-target binding affinity.
%We employ two real-world benchmarks containing various distribution shifts for graph OOD generalization to evaluate the effectiveness of our method.
% \begin{itemize}
%     \item \textbf{GOOD} is a systematic and comprehensive graph OOD benchmark, offering detailed distributions partition across various types of graphs. For the graph classification task, we selected three distinct datasets: (1) GOOD-HIV, a molecular graph dataset with the task of binary classification to predict whether a molecule can inhibit HIV; (2) GOOD-CMNIST, which consists of graphs representing hand-written digits transformed from the MNIST database using superpixel techniques; and (3) GOOD-Motif, a synthetic dataset where each graph is formed by connecting a base graph with a motif, where the motif alone determines the label.
%     \item \textbf{DrugOOD} is an OOD benchmark designed specifically for AI-driven drug discovery, where the data consists of molecular graphs. DrugOOD includes three basis of distribution shift: scaffold, size, and assay, and applies these to two measurements (IC50 and EC50). The benchmark contains six datasets, and all of them are tasked with predicting drug-target binding affinity, framed as a binary classification problem.
% \end{itemize}

\textbf{Baselines}.  For a more comprehensive comparison, we evaluate our method against ERM and two categories of OOD baselines: (1) Traditional OOD approaches that can also be applied to Euclidean data, such as Coral, IRM and VREx; and (2) graph-specific OOD generalization methods, including environment-based approaches like MoleOOD, CIGA, GIL, GREA and causal explanations based: Disc and DIR, along with novel model architecture like CAL and GSAT .

\textbf{Implementation Details}. To ensure fairness, we adopt the same experimental setup as iMold across two benchmarks. For molecular datasets with edge features, we use a three-layer GIN with a hidden dimension of 300, while for non-molecular graphs, we employ a four-layer GIN with a hidden dimension of 128. Prototype updating is fixed with a hyperparameter of 0.99, and we use the Adam optimizer for model parameter updates. The projector is a two-layer MLP with a hidden dimension set to half that of the GIN encoder. All baselines use the optimal parameters from their original papers. Additional hyperparameter details can be found in Appendix 2.

\subsection{main results}

\textbf{Q: Whether our methods achieves the best performance on the OOD generalization on these two benchmarks?} 
Yes, our method integrates hyperspherical space and invariant learning by optimizing the proposed objective function, ensuring the invariance of representations without relying on environmental information, while simultaneously enhancing separability

 \noindent$\rhd$ \textsf{State-of-the-art results.}
Table \ref{table_1} and Table \ref{table_2} present the experimental results on GOOD and DrugOOD benchmark. Our method achieves the state-of-the-art performance on 10 out of 11 datasets, securing second place on the remaining dataset. The average improvements against the previous SOTA are $4.87\%$ on GOOD and $1.68\%$ on DrugOOD. Our method consistently outperforms other baselines in terms of average performance across various data shifts, demonstrating its superior ability to achieve environment invariance. Moreover, our model achieves the best results in both binary and multi-class tasks, highlighting the strength of the multi-prototype-based classification approach.

 \noindent$\rhd$ \textsf{Environment-based methods fail.}
Among all baselines, environment-based methods only achieve the best performance on 5 datasets, while other methods perform best on the remaining datasets. Notably, general OOD methods still achieve the best results on three of these datasets. These observations suggest that environment-based methods are limited by the challenge of accurately defining environmental information in graph data, leading to a discrepancy between theoretical expectations and experimental results. In contrast, the performance of general OOD methods suggests that, even without specific environmental information for graphs, OOD generalization can still be achieved under certain conditions. 
\subsection{Ablation Experiment}
\textbf{Q: Whether each module in PGR-MOOD contribute to achieve effective OOD generalization?} Yes, we conduct experiments on three datasets to verify the role of our proposed loss constraint $\mathcal{L}_{\mathrm{inv}}$, $\mathcal{L}_{\mathrm{sep}}$, and the component of our model: projector and weight pruning technique. The results are shown in Table~\ref{ablation}.

\noindent$\rhd$ \textsf{Ablation on $\mathcal{L}_{\mathrm{inv}}$ and $\mathcal{L}_{\mathrm{sep}}$.}
 % \begin{document}
 We remove $\mathcal{L}_{\mathrm{inv}}$ and $\mathcal{L}_{\mathrm{sep}}$ in the Eq. (\ref{eq: target2}) respectively to explore their impacts on the performance of OOD generalization. The experimental results demonstrate a clear fact: merely optimizing  for invariance (w/o $\mathcal{L}_{\mathrm{sep}}$) or separability (w/o $\mathcal{L}_{\mathrm{inv}}$) weakens the OOD generalization ability of our model, especially for the multiclass classification task. This provides strong evidence that ensuring both invariance and separability is a sufficient and necessary condition for effective out-of-distribution generalization in graph learning.

 \noindent$\rhd$ \textsf{Ablation on projector and multi-prototype.}
 % \begin{document}
We conducted ablation studies by removing the projector and setting the number of prototypes to one to assess their impact on performance. The results demonstrate the necessity of both components. For the projector, as it projects the invariant features into the hyperspherical space, and the optimization of Eq. (\ref{eq: target2}) in the hyperspherical space cannot be completed if without it, even leading worse results than ERM. Similarly, the absence of multiple prototypes blurs the decision boundaries between classes, which in turn affects the calculation of the loss function $\mathcal{L}_{\mathrm{sep}}$, preventing the guarantee of inter-class separability.

 \noindent$\rhd$ \textsf{Ablation on updating and weight pruning.}
 % \begin{document}
We removed the prototype-related weight calculations and weight pruning operations separately. Experimental results show that proper weighting is essential for ensuring the correct alignment between representations and their corresponding prototypes. Without these techniques, the prototypes degrade into the average representation of all samples in the class, failing to maintain classification performance in OOD scenarios.

\subsection{Hyperparameter analysis}
 \noindent$\rhd$ \textsf{Analysis of $K$.}
 To investigate the effect of the number of prototypes on model performance, we vary $k$ from 2 to 5 and present the experimental results in Fig. \ref{hyper_p}. We observe that the best performance is achieved when the number of prototypes is approximately twice the number of classes (e.g., 2 or 3 for GOOD-HIV, and 5 or 6 for GOOD-Motif). Deviating from this optimal range, either too many or too few prototypes negatively impacts the final performance.
 
  \noindent$\rhd$ \textsf{Analysis of $\beta$.}
  To investigate the effect of the coefficient $\beta$ for $\mathcal{L}_{\mathrm{inv}}$ on model performance, we vary $\beta$ within {0.01, 0.05, 0.1, 0.2, 0.3} and present the results in Fig. \ref{hyper_a}. We observe that a small $\beta$ (e.g., 0.01, 0.05) hampers the model’s ability to effectively learn invariant features, while selecting a moderate $\beta$ (0.1) leads to the best performance.

\subsection{Analysis of the hyperspherical Space}
\textbf{Q: Whether hyperspherical Spaces are more separable than ordinary latent Spaces} Yes, the visualization shows the advantage of hyperspherical space over traditional latent space.

To further validate the advantage of hyperspherical latent space over traditional latent spaces, we visualized the invariant representation 
$\hat{\vz}_{inv}$ in both the training set (ID) and the test set (OOD) after achieving the best score on the validation set (ID). Using T-SNE, we visualize the representation on GOODHIV-Scaffold using T-sne, as shown in Figure \ref{t1}. For comparison, we also visualized the invariant representations learned by the state-of-the-art method, CIGA, as shown in Figure \ref{t2}. It is evident that our method produces more separable invariant representations, while also exhibiting tighter clustering for samples of the same class, indicating successful capture of environment-invariant features. In contrast, while CIGA also achieves some degree of intra-class compactness, its lower separability hampers its overall performance.

In addition, we reveal the characteristics of prototypes by visualizing samples that exhibit the highest similarity to them. As shown in Figure \ref{v_prototype}, prototypes from different classes capture distinct invariant subgraphs, ensuring a strong correlation with their respective labels. Furthermore, within the same category, different prototypes encapsulate samples with varying environmental subgraphs. This effectively validates the association between multi-prototype learning and environmental adaptability.
\begin{figure*}[t!] \label{v_prototype}
\centering    
\includegraphics[scale=0.39]{3_method/sx_prototype.pdf}
\caption{In the case of the DrugOOD-IC50-assay (binary classification task), we set up three prototypes for each class and visualized the closest example to it. }  
\label{fig:intro} 
\end{figure*}

\begin{table}[ht] \label{table_1}
\centering
\caption{Performance of various methods on IC50 and EC50 tasks.}
\begin{tabular}{l|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{IC50} $\uparrow$} & \multicolumn{3}{c}{\textbf{EC50} $\uparrow$} \\ 
 & \textbf{Assay} & \textbf{Scaffold} & \textbf{Size} & \textbf{Assay} & \textbf{Scaffold} & \textbf{Size} \\ \hline
ERM & 70.61 (0.75) & 67.54 (0.42) & 66.10 (0.31) & 65.27 (2.39) & 65.02 (1.10) & 65.17 (0.32) \\ 
IRM & 71.15 (0.57) & 67.22 (0.62) & \underline{67.58 (0.58)} & 67.77 (2.71) & 63.86 (1.36) & 59.19 (0.83) \\ 
VREx & 70.98 (0.77) & 68.02 (0.43) & 65.67 (0.19) & 69.84 (1.88) & 62.31 (0.96) & \underline{65.89 (0.83)} \\ 
Coral & 71.28 (0.91) & 68.36 (0.61) & 67.53 (0.32) & 72.08 (2.80) & 64.83 (1.64) & 58.47 (0.43) \\ \hline
MoleOOD & 71.62 (0.50) & 68.58 (1.14) & 67.22 (0.96) & 72.69 (4.16) & 65.78 (1.47) & 64.11 (1.04) \\ 
CIGA & \underline{71.86 (1.37)} & \textbf{69.14 (0.70)} & 66.99 (1.40) & 69.15 (5.79) & \underline{67.32 (1.35)} & 65.60 (0.82) \\ 
GIL & 70.66 (1.75) & 67.81 (1.03) & 66.23 (1.98) & 70.25 (5.79) & 63.95 (1.17) & 64.91 (0.76) \\ 
GREA & 70.23 (1.17) & 67.20 (0.77) & 66.09 (0.56) & 74.17 (1.47) & 65.84 (1.35) & 61.11 (0.46) \\  \hline
DIR & 69.84 (1.41) & 66.33 (0.65) & 62.92 (1.89) & 65.81 (2.93) & 63.76 (3.22) & 61.56 (4.23) \\ 
DisC & 61.40 (2.56) & 62.70 (2.11) & 64.43 (0.60) & 63.71 (5.56) & 60.57 (2.27) & 57.38 (2.48) \\ \hline
GSAT & 70.59 (0.43) & 66.94 (1.43) & 64.53 (0.51) & 73.82 (2.62) & 62.65 (1.79) & 62.65 (1.79) \\ 
CAL & 70.09 (1.03) & 65.90 (1.04) & 64.42 (0.50) & \underline{74.54 (1.48)} & 65.19 (0.87) & 61.21 (1.76) 
\\ \hline
Ours & \textbf{72.96 (1.21)} & \underline{68.62 (0.78)} & \textbf{68.06 (0.55)} & \textbf{78.08 (0.54)} & \textbf{68.34 (0.61)} & \textbf{68.11 (0.58)} \\ \hline
\end{tabular}
\end{table}

% \end{document}
\begin{table}[htbp] \label{table_2}
\centering
\begin{tabular}{l|cc|c|cc}
\toprule
           & \multicolumn{2}{c|}{GOOD-Motif} & \multicolumn{1}{c|}{GOOD-CMNIST} & \multicolumn{2}{c}{GOOD-HIV} \\
           & basis         & size          & color         & scaffold      & size \\
\midrule
ERM        & 60.93(2.11)  & 46.63(7.12)   & 26.64(2.37)   & 69.55(2.39)   & 59.19(2.29)\\
IRM        & 64.94(4.85)   & 54.52(3.27)   & 29.63(2.06)   & 70.17(2.78)   & 59.94(1.59)\\
VREX       & 61.59(6.58)   & \underline{55.85(9.42)}   & 27.13(2.90)   & 69.34(3.54)   & 58.49(2.28)\\
Coral      & 61.95(4.36)  & 55.80(4.05)   & 29.21(6.87)   & 70.69(2.25)   & 59.39(2.90)\\
\midrule
MoleOOD      & -  & -   & -  & 69.39(3.43)   & 58.63(1.78)\\
CIGA       & 67.81(2.42)   & 51.87(5.15)   & 25.06(3.07)   & 69.40(1.97)   & \underline{61.81(1.68)}\\
GIL      & 65.30(3.02)   & 54.65(2.09)   & 31.82(4.24)   & 68.59(2.11)   & 60.97(2.88)\\
GREA      & 59.91(2.74)   & 47.36(3.82)   & 22.12(5.07)   & \underline{71.98(2.87)}   & 60.11(1.07)\\
\midrule
DIR        & 64.39(2.02)   & 43.11(2.78)   & 22.53(2.56)   & 68.44(2.51)   & 57.67(3.75)\\
DisC       & 65.08(5.06)  & 42.23(4.20)   & 23.53(0.67)   & 58.85(7.26)  & 49.33(3.84)         \\ 
\midrule
GSAT       & 62.27(8.79)   & 50.03(5.71)   & \underline{35.02(2.78)}   & 70.07(1.76)   & 60.73(2.39)\\
CAL       & \underline{68.01(3.27)}   & 47.23(3.01)   & 27.15(5.66)   & 69.12(1.10)   & 59.34(2.14)\\
\midrule
Ours     & \textbf{76.23(4.89)} & \textbf{58.43(3.15)} & \textbf{41.29(3.85)} & \textbf{73.94(1.77)} & \textbf{66.84(1.09)}\\ \bottomrule
\end{tabular}
\caption{This is scm}
\end{table}

% \begin{table*}[ht]\tiny
% \centering
% \begin{tabular}{l|ccc|ccc|cc|c|cc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{IC50} $\uparrow$} & \multicolumn{3}{c}{\textbf{EC50} $\uparrow$} & \multicolumn{2}{c|}{GOOD-Motif} & \multicolumn{1}{c|}{GOOD-CMNIST} & \multicolumn{2}{c}{GOOD-HIV} \\ 
%  & Assay & Scaffold & Size & Assay & Scaffold & Size & basis  & size & color  & scaffold  & size \\ 
% \hline
% ERM & 70.61 (0.75) & 67.54 (0.42) & 66.10 (0.31) & 65.27 (2.39) & 65.02 (1.10) & 65.17 (0.32) & 60.93(2.11)  & 56.63(7.12)   & 26.64(2.37)   & 69.55(2.39)   & 59.19(2.29)\\ 
% IRM & 71.15 (0.57) & 67.22 (0.62) & 67.58 (0.58) & 67.77 (2.71) & 63.86 (1.36) & 59.19 (0.83) & 64.94(4.85)   & 54.52(3.27)   & 29.63(2.06)   & 70.17(2.78)   & 59.94(1.59)\\
% VREx & 70.98 (0.77) & 68.02 (0.43) & 65.67 (0.19) & 69.84 (1.88) & 62.31 (0.96) & 60.19 (0.73) & 61.59(6.58)   & 55.85(9.42)   & 27.13(2.90)   & 69.34(3.54)   & 58.49(2.28)\\ 
% Coral & 71.28 (0.91) & 68.36 (0.61) & 67.53 (0.32) & 72.08 (2.80) & 64.83 (1.64) & 58.47 (0.43) & 61.95(4.36)  & 55.80(4.05)   & 29.21(6.87)   & 70.69(2.25)   & 59.39(2.90)\\
% \hline
% MoleOOD & 71.62 (0.50) & 68.58 (1.14) & 67.22 (0.96) & 72.69 (4.16) & 65.78 (1.47) & 65.51 (1.24) & -    & - & -    & - & -   \\ 
% CIGA & 71.86 (1.37) & \textbf{69.14 (0.70)} & 66.99 (1.40) & 69.15 (5.79) & 67.32 (1.35) & 65.60 (0.82) & 67.81(2.42)   & 51.87(5.15)   & 25.06(3.07)   & 69.40(1.97)   & 61.81(1.68) \\ 
% GIL & 70.66 (1.75) & 67.81 (1.03) & 66.23 (1.98) & 70.25 (5.79) & 63.95 (1.17) & 64.91 (0.76) & -    & - & -    & - & -   \\ 
% GREA & 70.23 (1.17) & 67.20 (0.77) & 66.09 (0.56) & 74.17 (1.47) & 65.84 (1.35) & 61.11 (0.46) & -    & - & -    & - & -    \\  
% \hline
% DIR & 69.84 (1.41) & 66.33 (0.65) & 62.92 (1.89) & 65.81 (2.93) & 63.76 (3.22) & 61.56 (4.23) & 64.39(2.02)   & 43.11(2.78)   & 22.53(2.56)   & 68.44(2.51)   & 57.67(3.75) \\ 
% DisC & 61.40 (2.56) & 62.70 (2.11) & 64.43 (0.60) & 63.71 (5.56) & 60.57 (2.27) & 57.38 (2.48) & -    & - & -    & - & -   \\ 
% \hline
% GSAT & 70.59 (0.43) & 66.94 (1.43) & 64.53 (0.51) & 73.82 (2.62) & 62.65 (1.79) & 62.65 (1.79)    & 62.27(8.79)   & 50.03(5.71)   & 35.02(2.78)   & 70.07(1.76)   & 60.73(2.39) \\ 
% CAL & 70.09 (1.03) & 65.90 (1.04) & 64.42 (0.50) & 74.54 (1.48) & 65.19 (0.87) & 61.21 (1.76) & -    & - & -    & - & -    \\ 
% \hline
% Ours & \textbf{72.96 (1.21)} & 68.62 (0.78) & \textbf{68.06 (0.55)} & \textbf{78.08 (0.54)} & \textbf{68.34 (0.61)} & \textbf{68.11 (0.58)} \\ \hline
% \end{tabular}
% \caption{Performance of various methods on IC50 and EC50 tasks.}
% \end{table*}


\begin{table}[ht]\label{ablation}
\centering
\begin{tabular}{lccc}
\toprule
 Mothod &IC50-size &HIV-scaffold &CMNIST-color \\
\midrule
Ours & \textbf{68.06 (0.55)} & \textbf{73.94 (1.77)} & \textbf{41.29 (3.85)}  \\
ERM & 66.10 (0.31) & 69.55 (2.39) & 26.64 (2.37)  \\
\midrule

w/o $\mathcal{L}_{inv}$ & 67.09 (0.65) & 70.61 (1.52) & 37.86 (3.44)  \\
w/o $\mathcal{L}_{sep}$ & 66.21 (0.37)  & 71.06 (1.56) & 37.53 (2.18) \\
\midrule
w/o projector & 51.96 (2.54) & 65.78 (3.57) & 21.05 (4.89) \\
w/o multi-prototype & 57.64 (1.02) & 62.11 (1.95) & 20.58 (3.78)  \\
\midrule
w/o updating & 54.14 (1.22) & 67.89 (1.84) & 38.95 (3.01)  \\
w/o weight pruning & 67.64 (1.02) & 71.11 (1.95) & 40.58 (3.78) \\
\bottomrule
\end{tabular}
\caption{Experimental results on GOOD-HIV-Scaffold and GOOD-PCBA-Size datasets.}
\end{table}



\begin{figure*}[h]
\centering 
\subfigure { 
\includegraphics[width=0.23\columnwidth]{K_hiv.pdf} 
}
\subfigure{ 
\includegraphics[width=0.23\columnwidth]{K_motif.pdf} 
}
\subfigure { 
\includegraphics[width=0.23\columnwidth]{K_a.pdf}
}
\subfigure { 
\includegraphics[width=0.23\columnwidth]{K_a_motif.pdf}
}
\caption{Left, Middle:} 
\label{hyperparameter}
\vspace{-1pt}
\end{figure*}

\begin{figure*}[h]
\centering 
\subfigure[CIGA] { 
\includegraphics[width=0.4\textwidth]{imold.pdf} \label{t1}
}
\subfigure[Ours] { 
\includegraphics[width=0.4\textwidth]{my(1).pdf} \label{t2}
}

\caption{Left, Middle:} 
\label{t-sne}
\vspace{-1pt}
\end{figure*}

% \begin{figure}[!ht] \label{hyper_p}   
% 					\centering            % 前面说过，图片放置在中间
% 					 % 第一张子图的下标（注意：注释要写在[]中括号内）
% 					{
% 						\label{apha}\includegraphics[width=0.25\textwidth,height=0.13\textheight]{K.pdf}
						
% 					}\hspace{2mm}
				
% 					{
% 						\label{length}\includegraphics[width=0.25\textwidth,height=0.13\textheight]{K_motif.pdf}
% 					}
					
% 					 \vspace{-10pt}
% 					\caption{ Analysis of Hyper-Parameters of our method on two GOOD datasets.}    % 整个图片的说明，注释写在{}内
% 					\label{figinfluence}            % 整个图片的标签编号，注意这里跟
     
% \end{figure}
% \begin{figure}[!ht] \label{hyper_a}   
% 					\centering            % 前面说过，图片放置在中间
% 					 % 第一张子图的下标（注意：注释要写在[]中括号内）
% 					{
% 						\label{apha}\includegraphics[width=0.25\textwidth,height=0.13\textheight]{K_a.pdf}
						
% 					}\hspace{2mm}
				
% 					{
% 						\label{length}\includegraphics[width=0.25\textwidth,height=0.13\textheight]{K_motif_a.pdf}
% 					}
					
% 					 \vspace{-10pt}
% 					\caption{ Analysis of Hyper-Parameters of our method on two GOOD datasets.}    % 整个图片的说明，注释写在{}内
% 					\label{figinfluence}            % 整个图片的标签编号，注意这里跟
     
% \end{figure}

==> tables/main.tex <==
\begin{table*}[h!]
\caption{Performance comparison in terms of average accuracy (standard deviation) on GOOD benchmark.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|c|cc|cc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{GOOD-Motif}} & \multicolumn{1}{c|}{\textbf{GOOD-CMNIST}} & \multicolumn{2}{c|}{\textbf{GOOD-HIV}} & \multicolumn{2}{c|}{\textbf{GOOD-PCBA}} & \multicolumn{1}{c|}{\textbf{GOOD-SST}} & \multicolumn{1}{c}{\textbf{Spmotif}} \\
 & \textbf{basis} & \textbf{size} & \textbf{color} & \textbf{scaffold} & \textbf{size} & \textbf{scaffold} & \textbf{size} & \textbf{length} & \textbf{basis} \\
\midrule
ERM & 60.93 (2.11) & 46.63 (7.12) & 26.64 (2.37) & 69.55 (2.39) & 59.19 (2.29) & 21.93 (0.74) & 15.60 (0.55) & 26.64 (2.37) & 49.64 (2.39) \\
IRM & 64.94 (4.85) & {54.52 (3.27)} & 29.63 (2.06) & 70.17 (2.78) & 59.94 (1.59) & 22.37(0.43) & 15.82(0.52) & 29.63 (2.06) & 45.68(4.88) \\
VREX & 61.59 (6.58) & {55.85 (9.42)} & 27.13 (2.90) & 69.34 (3.54) & 58.49 (2.28) & 21.65(0.82) & 15.85(0.47) & 27.13 (2.90) & 48.86(9.69) \\
Coral & 61.95 (4.36) & 55.80 (4.05) & 29.21 (6.87) & 70.69 (2.25) & 59.39 (2.90) & 22.00(0.46) & 16.88(0.58) & 29.21 (6.87) & 70.69 (2.25) \\
\textcolor{red}{G-mixup} & \textcolor{red}{61.42 (2.05)} & \textcolor{red}{47.81 (6.98)} & \textcolor{red}{26.12 (2.51)} & \textcolor{red}{68.93 (2.41)} & \textcolor{red}{59.84 (2.33)} & - & - & - & - \\
\midrule
MoleOOD & - & - & - & 69.39 (3.43) & 58.63 (1.78) & 12.92(1.23) & 10.30(0.36) & - & - \\
CIGA & 67.81 (2.42) & 51.87 (5.15) & 25.06 (3.07) & 69.40 (1.97) & {61.81 (1.68)} & - & - & 25.06 (3.07) & 63.41 (7.38) \\
GIL & 65.30 (3.02) & 54.65 (2.09) & 31.82 (4.24) & 68.59 (2.11) & 60.97 (2.88) & - & - & 31.82 (4.24) & 68.59 (2.11) \\
GREA & 59.91 (2.74) & 47.36 (3.82) & 22.12 (5.07) & {71.98 (2.87)} & 60.11 (1.07) & 20.23(1.53) & 13.82(1.18) & 22.12 (5.07) & {71.98 (2.87)} \\
IGM & {74.69 (8.51)} & 52.01 (5.87) & 33.95 (4.16) & {71.36 (2.87)} & 62.54 (2.88) & 20.09(1.99) & 12.87(0.69) & 33.95 (4.16) & {71.36 (2.87)} \\
\midrule
DIR & 64.39 (2.02) & 43.11 (2.78) & 22.53 (2.56) & 68.44 (2.51) & 57.67 (3.75) & 23.82(0.89) & 16.80(1.17) & 22.53 (2.56) & 41.90(9.39) \\
DisC & 65.08 (5.06) & 42.23 (4.20) & 23.53 (0.67) & 58.85 (7.26) & 49.33 (3.84) & - & - & 23.53 (0.67) & 58.85 (7.26) \\
\midrule
GSAT & 62.27 (8.79) & 50.03 (5.71) & {35.02 (2.78)} & 70.07 (1.76) & 60.73 (2.39) & 20.18(0.74) & 13.52(0.90) & {35.02 (2.78)} & 70.07 (1.76) \\
CAL & {68.01 (3.27)} & 47.23 (3.01) & 27.15 (5.66) & 69.12 (1.10) & 59.34 (2.14) & 18.62(1.21) & 13.01(0.65) & 27.15 (5.66) & 69.12 (1.10) \\
iMoLD & - & - & - & \underline{72.05 (2.16)} & {62.86 (2.34)} & 22.58(0.67) & 18.21(1.10) & - & \underline{72.05 (2.16)} \\
\textcolor{black}{GALA} & \textcolor{black}{72.97 (4.28)} & \textcolor{black}{\textbf{60.82 (0.51)}} & \textcolor{black}{\underline{40.62 (2.11)}} & \textcolor{black}{71.22 (1.93)} & \textcolor{black}{\underline{65.29 (0.72)}} & 21.26(1.48) & 13.57 (0.88) & \textcolor{black}{\underline{40.62 (2.11)}} & \textcolor{black}{71.22 (1.93)} \\
\textcolor{black}{EQuAD} & \textcolor{black}{\underline{75.46 (4.35)}} & \textcolor{black}{55.10 (2.91)} & \textcolor{black}{{40.29 (3.95)}} & \textcolor{black}{71.49 (0.67)} & \textcolor{black}{{64.09 (1.08)}} & \textcolor{black}{\underline{23.17 (0.80)}} & \textcolor{black}{17.61 (0.76)} & \textcolor{black}{{40.29 (3.95)}} & \textcolor{black}{71.49 (0.67)} \\
\textcolor{red}{HSE} & \textcolor{red}{74.62 (3.05)} & \textcolor{red}{54.03 (1.85)} & \textcolor{red}{39.17 (5.17)} & \textcolor{red}{70.85 (1.97)} & \textcolor{red}{63.41 (2.14)} & 17.41(0.83) & 17.53 (0.76) & {38.95 (2.97)} & 69.12 (1.10) \\
\textcolor{red}{LIRS} & \textcolor{red}{74.31 (4.66)} & \textcolor{red}{53.78 (2.17)} & \textcolor{red}{39.02 (3.78)} & \textcolor{red}{70.54 (0.51)} & \textcolor{red}{63.10 (1.21)} & 20.98(1.57) & 19.11(1.34) & - & \underline{72.05 (2.16)} \\
\midrule
\ourmethod & \textbf{76.23 (4.89)} & \underline{58.43 (3.15)} & \textbf{41.29 (3.85)} & \textbf{73.94 (1.77)} & \textbf{66.84 (1.09)} & \textbf{25.73 (0.79)} & \underline{58.43 (3.15)} & \textbf{41.29 (3.85)} & \textbf{73.94 (1.77)} \\
\bottomrule
\end{tabular}
\label{tab:merged_good}
}
\end{table*}

==> tables/main_good_full.tex <==
\begin{table*}[h!] 

\caption{Performance comparison in terms of average accuracy (standard deviation) on GOOD benchmark.}
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|cc|c|cc}
\toprule
\multirow{2}{*}{\textbf{Method}}           & \multicolumn{2}{c|}{\textbf{GOOD-Motif}} & \multicolumn{1}{c|}{\textbf{GOOD-CMNIST}} & \multicolumn{2}{c}{\textbf{GOOD-HIV}} \\
           & \textbf{basis}         & \textbf{size}          & \textbf{color}         & \textbf{scaffold}      & \textbf{size} \\
\midrule
ERM        & 60.93 (2.11)  & 46.63 (7.12)   & 26.64 (2.37)   & 69.55 (2.39)   & 59.19 (2.29)\\
IRM        & 64.94 (4.85)   & {54.52 (3.27)}   & 29.63 (2.06)   & 70.17 (2.78)   & 59.94 (1.59)\\
VREX       & 61.59 (6.58)   & {55.85 (9.42)}   & 27.13 (2.90)   & 69.34 (3.54)   & 58.49 (2.28)\\
Coral      & 61.95 (4.36)  & 55.80 (4.05)   & 29.21 (6.87)   & 70.69 (2.25)   & 59.39 (2.90)\\
\textcolor{red}{G-mixup}    & \textcolor{red}{61.42 (2.05)}  & \textcolor{red}{47.81 (6.98)}   & \textcolor{red}{26.12 (2.51)}  & \textcolor{red}{68.93 (2.41)}   & \textcolor{red}{59.84 (2.33)} \\
\midrule
MoleOOD      & -  & -   & -  & 69.39 (3.43)   & 58.63 (1.78)\\
CIGA       & 67.81 (2.42)   & 51.87 (5.15)   & 25.06 (3.07)   & 69.40 (1.97)   & {61.81 (1.68)}\\
GIL      & 65.30 (3.02)   & 54.65 (2.09)   & 31.82 (4.24)   & 68.59 (2.11)   & 60.97 (2.88)\\
GREA      & 59.91 (2.74)   & 47.36 (3.82)   & 22.12 (5.07)   & {71.98 (2.87)}   & 60.11 (1.07)\\
IGM    & {74.69 (8.51) }  & 52.01 (5.87)   & 33.95 (4.16)   & {71.36 (2.87)}   & 62.54 (2.88)\\
\midrule
DIR        & 64.39 (2.02)   & 43.11 (2.78)   & 22.53 (2.56)   & 68.44 (2.51)   & 57.67 (3.75)\\
DisC       & 65.08 (5.06)  & 42.23 (4.20)   & 23.53 (0.67)   & 58.85 (7.26)  & 49.33 (3.84)         \\ 
\midrule
GSAT       & 62.27 (8.79)   & 50.03 (5.71)   & {35.02 (2.78)}   & 70.07 (1.76)   & 60.73 (2.39)\\
CAL       & {68.01 (3.27)}   & 47.23 (3.01)   & 27.15 (5.66)   & 69.12 (1.10)   & 59.34 (2.14)\\
iMoLD      & - & - & -  & \underline{72.05 (2.16)}   & {62.86 (2.34)}\\
\textcolor{black}{GALA} & \textcolor{black}{72.97 (4.28)} & \textcolor{black}{\textbf{60.82 (0.51)}} & \textcolor{black}{\underline{40.62 (2.11)}} & \textcolor{black}{71.22 (1.93)}& \textcolor{black}{\underline{65.29 (0.72)}}\\
\textcolor{black}{EQuAD}      &\textcolor{black}{\underline{75.46 (4.35)}}   & \textcolor{black}{55.10 (2.91)}   & \textcolor{black}{{40.29 (3.95)}}   & \textcolor{black}{71.49 (0.67)}    &\textcolor{black}{{64.09 (1.08)}}     \\
\textcolor{red}{HSE}      &\textcolor{red}{74.62 (3.05)}   & \textcolor{red}{54.03 (1.85)}   & \textcolor{red}{39.17 (5.17)}   & \textcolor{red}{70.85 (1.97)}    &\textcolor{red}{63.41 (2.14)}  \\
\textcolor{red}{LIRS}      &\textcolor{red}{74.31 (4.66)}   & \textcolor{red}{53.78 (2.17) }   & \textcolor{red}{39.02 (3.78)}   & \textcolor{red}{70.54 (0.51)}    &\textcolor{red}{63.10 (1.21)}    \\
\midrule
\ourmethod     & \textbf{76.23 (4.89)} & \underline{58.43 (3.15)} & \textbf{41.29 (3.85)} & \textbf{73.94 (1.77)} & \textbf{66.84 (1.09)}\\ \bottomrule
\end{tabular}\label{tab:main_good}}
\end{table*}

\begin{table*}[h!] 

\caption{Performance comparison in terms of average accuracy (standard deviation) on GOOD benchmark.}
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|cc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}}           & \multicolumn{2}{c|}{\textbf{GOOD-PCBA}} & \multicolumn{1}{c|}{\textbf{GOOD-SST}} & \multicolumn{1}{c}{\textbf{Spmotif}} \\
           & \textbf{scaffold}         & \textbf{size}          & \textbf{length}         & \textbf{basis}      \\
\midrule
ERM        & 21.93 (0.74)  & 15.60 (0.55)   & 26.64 (2.37)   & 49.64 (2.39)   \\
IRM        & 22.37(0.43)   & 15.82(0.52)   & 29.63 (2.06)   & 45.68(4.88)  \\
VREX       & 21.65(0.82)   & 15.85(0.47)   & 27.13 (2.90)   & 48.86(9.69)   \\
Coral      & 22.00(0.46)  & 16.88(0.58)   & 29.21 (6.87)   & 70.69 (2.25)  \\
\midrule
MoleOOD      & 12.92(1.23)  & 10.30(0.36)   & -  & -    \\
CIGA       & -   & -   & 25.06 (3.07)   & 63.41 (7.38)   \\
GIL      & -   & -   & 31.82 (4.24)   & 68.59 (2.11)   \\
GREA      & 20.23(1.53)   & 13.82(1.18)   & 22.12 (5.07)   & {71.98 (2.87)}   \\
IGM    & 20.09(1.99)  & 12.87(0.69)   & 33.95 (4.16)   & {71.36 (2.87)}  \\
\midrule
DIR        & 23.82(0.89)   & 16.80(1.17)   & 22.53 (2.56)   & 41.90(9.39)   \\
DisC       & -  & -   & 23.53 (0.67)   & 58.85 (7.26)          \\ 
\midrule
GSAT       & 20.18(0.74)   & 13.52(0.90)   & {35.02 (2.78)}   & 70.07 (1.76)  \\
CAL       & 18.62(1.21)   & 13.01(0.65)   & 27.15 (5.66)   & 69.12 (1.10)   \\
GALA       & 21.26(1.48)   & 13.57 (0.88)   & {38.95 (2.97)}   & 69.12 (1.10)   \\
iMoLD      & 22.58(0.67) & 18.21(1.10) & -  & \underline{72.05 (2.16)}   \\
\textcolor{black}{GALA}  & 21.26(1.48)   & 13.57 (0.88) & \textcolor{black}{\underline{40.62 (2.11)}} & \textcolor{black}{71.22 (1.93)}\\
\textcolor{black}{EQuAD}      &\textcolor{black}{\underline{23.17 (0.80)}}   & \textcolor{black}{17.61 (0.76)}   & \textcolor{black}{{40.29 (3.95)}}   & \textcolor{black}{71.49 (0.67)}        \\
HSE       & 17.41(0.83)   & 17.53 (0.76)   & {38.95 (2.97)}   & 69.12 (1.10)   \\
LIRS      & 20.98(1.57) & 19.11(1.34) & -  & \underline{72.05 (2.16)}   \\
\midrule
\ourmethod     & \textbf{25.73 (0.79)} & \underline{58.43 (3.15)} & \textbf{41.29 (3.85)} & \textbf{73.94 (1.77)} \\ \bottomrule
\end{tabular}\label{tab:main_good}}
\end{table*}
